Active Learning For Repairable Hardware Systems With Partial Coverage

Identifying the optimal diagnostic test and hardware system instance to infer reliability characteristics using field data is challenging, especially when constrained by fixed budgets and minimal maintenance cycles. Active Learning (AL) has shown promise for parameter inference with limited data and budget constraints in machine learning/deep learning tasks. However, AL for reliability model parameter inference remains underexplored for repairable hardware systems. It requires specialized AL Acquisition Functions (AFs) that consider hardware aging and the fact that a hardware system consists of multiple sub-systems, which may undergo only partial testing during a given diagnostic test. To address these challenges, we propose a relaxed Mixed Integer Semidefinite Program (MISDP) AL AF that incorporates Diagnostic Coverage (DC), Fisher Information Matrices (FIMs), and diagnostic testing budgets. Furthermore, we design empirical-based simulation experiments focusing on two diagnostic testing scenarios: (1) partial tests of a hardware system with overlapping subsystem coverage, and (2) partial tests where one diagnostic test fully subsumes the subsystem coverage of another. We evaluate our proposed approach against the most widely used AL AF in the literature (entropy), as well as several intuitive AL AFs tailored for reliability model parameter inference. Our proposed AF ranked best on average among the alternative AFs across 6,000 experimental configurations, with respect to Area Under the Curve (AUC) of the Absolute Total Expected Event Error (ATEER) and Mean Squared Error (MSE) curves, with statistical significance calculated at a 0.05 alpha level using a Friedman hypothesis test.

==> overlapping_critical_difference_diagram.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \begin{tabular}{c|cc|}
%         % Column Labels
%         & \textbf{Column 1 Label} & \textbf{Column 2 Label} \\
%         \hline
%         % Row 1
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\tiny \textbf{Row 1 Label}}} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.050 k=1.300.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 2
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\tiny \textbf{Row 2 Label}}} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 3
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\tiny \textbf{Row 3 Label}}} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.45\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%     \end{tabular}
%     \caption{Overlapping}
%     \label{fig:cdoverlapping}
% \end{figure*}

% \begin{figure*}[htbp]
%     \centering
%     \begin{tabular}{c|cc|}
%         % Column Labels
%         & \textbf{\gls{ateer}} & \textbf{\gls{mse}} \\
%         \hline
%         % Row 1
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.1\) \\ \(k = 1.3\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.050 k=1.300.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.050 k=1.300.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 2
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.25\) \\ \(k = 2.0\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 3
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.5\) \\ \(k = 0.5\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_ATEER_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/overlap_cd/overlapping_MSE_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%     \end{tabular}
%     \caption{Overlapping configuration: the critical difference diagrams display the average ranks of the acquisition functions across various experiment realizations, considering combinations of diagnostic coverage coefficients, maintenance cycle frequency, and maintenance budget. For both \gls{ateer} and \gls{mse}, a lower rank indicates a better acquisition function.}
%     \label{fig:cdoverlapping}
% \end{figure*}

% \begin{figure}[h!]
%     \centering
%     \includegraphics{images/critical_difference_overlap.png}
%     \caption{Overlapping configuration: the critical difference diagrams display the average ranks of the acquisition functions across various experiment realizations, considering combinations of diagnostic coverage coefficients, maintenance cycle frequency, and maintenance budget. For both \gls{ateer} and \gls{mse}, a lower rank indicates a better acquisition function.}
%     \label{fig:cdoverlapping}
% \end{figure}

==> subset_critical_difference_diagram.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \begin{tabular}{c|cc|}
%         % Column Labels
%         & \textbf{\gls{ateer}} & \textbf{\gls{mse}} \\
%         \hline
%         % Row 1
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.1\) \\ \(k = 1.3\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_ATEER_alpha=0.050 k=1.300.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_MSE_alpha=0.050 k=1.300.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 2
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.25\) \\ \(k = 2.0\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_ATEER_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_MSE_alpha=0.062 k=2.000.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%         % Row 3
%         \multirow{3}{*}[5.5em]{\rotatebox[origin=c]{90}{\tiny \textbf{\parbox{2.2cm}{\(\lambda = 0.5\) \\ \(k = 0.5\)}}}} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_ATEER_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} &
%         \begin{minipage}[t]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{images/subset_cd/subset_MSE_alpha=0.707 k=0.500.png} % \caption{Plot 6 Caption}
%         \end{minipage} \\
%         \hline
%     \end{tabular}
%     \caption{Subset configuration: the critical difference diagrams display the average ranks of the acquisition functions across various experiment realizations, considering combinations of diagnostic coverage coefficients, maintenance cycle frequency, and maintenance budget. For both \gls{ateer} and \gls{mse}, a lower rank indicates a better acquisition function.}
%     \label{fig:cdsubset}
% \end{figure*}
